Advanced Strategies for Uncertainty-Guided Live Measurement Sequencing in Fast, Robust SAR ADC Linearity Testing

This paper builds on our Uncertainty-Guided Live Measurement Sequencing (UGLMS) method. UGLMS is a closed-loop test strategy that adaptively selects SAR ADC code edges based on model uncertainty and refines a behavioral mismatch model in real time via an Extended Kalman Filter (EKF), eliminating full-range sweeps and offline post-processing. We introduce an enhanced UGLMS that delivers significantly faster test runtimes while maintaining estimation accuracy. First, a rank-1 EKF update replaces costly matrix inversions with efficient vector operations, and a measurement-aligned covariance-inflation strategy accelerates convergence under unexpected innovations. Second, we extend the static mismatch model with a low-order carrier polynomial to capture systematic nonlinearities beyond pure capacitor mismatch. Third, a trace-based termination adapts test length to convergence, preventing premature stops and redundant iterations. Simulations show the enhanced UGLMS reconstructs full Integral- and Differential-Non-Linearity (INL/DNL) in just 36 ms for 16-bit and under 70 ms for 18-bit ADCs (120 ms with the polynomial extension). Combining the faster convergence from covariance inflation with reduced per-iteration runtime from the rank-1 EKF update, the method reaches equal accuracy 8x faster for 16-bit ADCs. These improvements enable real-time, production-ready SAR ADC linearity testing.

==> Plots/NN_HistComparison/HistComparison_DNL.tex <==
\begin{tikzpicture}
\begin{axis}[
    % xlabel={ADC Code},
    ylabel={DNL $[LSB]$},
    grid=major,
    ymin=-1.05,
    ymax=1.05,
    xmin=0,
    xmax=4096,
    xtick distance=1024,
    xticklabel style={/pgf/number format/1000 sep=},
    width=\linewidth,
    height=0.65\linewidth,
    legend pos=south east,
    legend cell align={right},
    legend style={draw=none, font=\footnotesize},
    legend image post style={line width=1pt}, % Make legend lines thicker
]
\addplot[blue] table {Plots/HistComparison/hist_est_dnl.dat};
\addlegendentry{Hist DNL};
\addplot[red] table {Plots/HistComparison/est_dnl.dat};
\addlegendentry{Estimated DNL};
        
\end{axis}
\end{tikzpicture}

==> Plots/NN_HistComparison/HistComparison_INL.tex <==
\begin{tikzpicture}
\begin{axis}[
    % xlabel={ADC Code},
    ylabel={INL $[LSB]$},
    ylabel style={yshift=8pt},
    grid=major,
    ymin=-1.35,
    ymax=1.35,
    xmin=0,
    xmax=4096,
    xmajorticks=false, 
    % xtick distance=1024,
    % xticklabel style={/pgf/number format/1000 sep=},
    width=0.96\linewidth,
    height=0.65\linewidth,
    legend pos=north east,
    legend cell align={right},
    legend style={draw=none, font=\footnotesize},
    legend image post style={line width=1pt}, % Make legend lines thicker
]
\addplot[cyan] table {Plots/HistComparison/hist_est_inl.dat};
\addlegendentry{RHT (128HPC)};
\addplot[red] table {Plots/HistComparison/est_inl.dat};
\addlegendentry{Proposed Method};
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    % xlabel={ADC Code},
    ylabel={DNL $[LSB]$},
    grid=major,
    ymin=-1.05,
    ymax=1.05,
    xmin=0,
    xmax=4096,
    xtick distance=1024,
    xticklabel style={/pgf/number format/1000 sep=},
    width=0.96\linewidth,
    height=0.65\linewidth,
    legend pos=south east,
    legend cell align={right},
    legend style={draw=none, font=\footnotesize},
    legend image post style={line width=1pt}, % Make legend lines thicker
]
\addplot[cyan] table {Plots/HistComparison/hist_est_dnl.dat};
\addlegendentry{RHT (128HPC)};
\addplot[red] table {Plots/HistComparison/est_dnl.dat};
\addlegendentry{Proposed Method};
\end{axis}
\end{tikzpicture}

==> Plots/NN_SingleRun_DNL/SingleRun_DNL.tex <==
\begin{tikzpicture}
\begin{axis}[
    % xlabel={ADC Code},
    ylabel={DNL $[LSB]$},
    grid=major,
    ymin=-1.05,
    ymax=1.05,
    xmin=0,
    xmax=4096,
    % xtick distance=1024,
    % xticklabel style={/pgf/number format/1000 sep=},
    xmajorticks=false,
    width=\linewidth,
    height=0.65\linewidth,
    legend pos=south east,
    legend cell align={right},
    legend style={draw=none, font=\footnotesize},
    legend image post style={line width=1pt}, % Make legend lines thicker
]
\addplot[blue] table {Plots/SingleRun_DNL/true_dnl.dat};
\addlegendentry{Ground Truth};
\addplot[red] table {Plots/SingleRun_DNL/est_dnl.dat};
\addlegendentry{Proposed Method};
        
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    xlabel={ADC Code},
    ylabel={$\Delta$DNL $[LSB]$},
    grid=major,
    ymin=-0.15,
    ymax=0.15,
    xmin=0,
    xmax=4096,
    xtick distance=1024,
    xticklabel style={/pgf/number format/1000 sep=},
    ytick distance=0.1,
    width=\linewidth,
    height=0.4\linewidth,    
]
\addplot[blue] table {Plots/SingleRun_DNL/diff_dnl.dat};

\end{axis}
\end{tikzpicture}

==> Plots/NN_SingleRun_INL/SingleRun_INL.tex <==
\begin{tikzpicture}
\begin{axis}[
    % xlabel={ADC Code},
    ylabel={INL $[LSB]$},
    ylabel style={yshift=8pt},
    grid=major,
    ymin=-1.35,
    ymax=1.35,
    xmin=0,
    xmax=4096,
    % xtick distance=1024,
    % xticklabel style={/pgf/number format/1000 sep=},
    xmajorticks=false,
    width=\linewidth,
    height=0.65\linewidth,
    legend pos=north east,
    legend cell align={right},
    legend style={draw=none, font=\footnotesize},
    legend image post style={line width=1pt}, % Make legend lines thicker
]
\addplot[blue] table {Plots/SingleRun_INL/true_inl.dat};
\addlegendentry{Ground Truth};
\addplot[red] table {Plots/SingleRun_INL/est_inl.dat};
\addlegendentry{Proposed Method};
        
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    xlabel={ADC Code},
    ylabel={$\Delta$INL $[LSB]$},
    grid=major,
    ymin=-0.15,
    ymax=0.15,
    xmin=0,
    xmax=4096,
    xtick distance=1024,
    xticklabel style={/pgf/number format/1000 sep=},
    ytick distance=0.1,
    width=\linewidth,
    height=0.4\linewidth,    
]
\addplot[blue] table {Plots/SingleRun_INL/diff_inl.dat};

\end{axis}
\end{tikzpicture}

==> Plots/SingleRun_Group/SingleRun_Group.tex <==
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=1 by 4,
        vertical sep=4pt,
        horizontal sep=0cm,
    },
    width=0.78\linewidth,
    height=0.5\linewidth,
    scale only axis=true,
    xmin=0, xmax=4096,
    grid=major,
    legend style={draw=none, font=\footnotesize},
    legend cell align={right},
    legend image post style={line width=1pt},
]

% Top-left: INL
\nextgroupplot[
    ylabel={INL $[LSB]$},
    ylabel style={yshift=8.5pt},
    ymin=-1.0, ymax=2.1,
    xtick distance=1024,
    xmajorticks=false,
    legend pos=north east,
]
\addplot[blue] table {Plots/SingleRun_Group/true_inl.dat};
\addlegendentry{Ground Truth};
\addplot[red] table {Plots/SingleRun_Group/est_inl.dat};
\addlegendentry{Proposed Method};
\addplot[cyan] table {Plots/SingleRun_Group/poly_inl.dat};
\addlegendentry{Quadratic Carrier};

% Bottom-left: ΔINL
\nextgroupplot[
    % xlabel={ADC Code},
    ylabel={$ \Delta $INL $[LSB]$},
    ymin=-0.15, ymax=0.15,
    xmajorticks=false,
    xtick distance=1024,
    % xticklabel style={/pgf/number format/1000 sep=},
    ytick distance=0.1,
    height=0.2\linewidth,
]
\addplot[blue] table {Plots/SingleRun_Group/diff_inl.dat};

% Top-right: DNL
\nextgroupplot[
    ylabel={DNL $[LSB]$},
    ymin=-1.05, ymax=1.05,
    xtick distance=1024,
    xmajorticks=false,
    legend pos=south east,
]
\addplot[blue] table {Plots/SingleRun_Group/true_dnl.dat};
\addlegendentry{Ground Truth};
\addplot[red] table {Plots/SingleRun_Group/est_dnl.dat};
\addlegendentry{Proposed Method};

% Bottom-right: ΔDNL
\nextgroupplot[
    xlabel={ADC Code},
    ylabel={$ \Delta $DNL $[LSB]$},
    ymin=-0.15, ymax=0.15,
    xtick distance=1024,
    xticklabel style={/pgf/number format/1000 sep=},
    ytick distance=0.1,
    height=0.2\linewidth,
]
\addplot[blue] table {Plots/SingleRun_Group/diff_dnl.dat};

\end{groupplot}

\end{tikzpicture}

==> Plots/StatisticalAnalysisINL/StatisticalAnalysisINL.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=\linewidth,
    % Axis only left and bottom without arrows
    axis lines=left,
    axis line style={-},
    % Axis limits
    xmin=-4, xmax=4,
    ymin=-4, ymax=4,
    restrict x to domain=-4.5:4.5,
    restrict y to domain=-4.5:4.5,
    % Axis labels
    xlabel={{Reference INL $[LSB_{16}]$}},
    ylabel={{INL from proposed method $[LSB_{16}]$}},
    % Ticks every 1
    xtick distance=1,
    ytick distance=1,
    % Grid only at ±2
    extra x ticks={-2,2},
    extra y ticks={-2,2},
    extra x tick style={grid=major},
    extra y tick style={grid=major},
    % General grid style
    grid style={gray!50, line width=0.5pt},
    tick align=inside,
    axis on top,
    % clip=true,
    % legend pos=north east,
    legend cell align={right},
    legend style={at={(0.6, 0.26)}, anchor=south, draw=none, fill=none, font=\footnotesize},
    legend image post style={mark size=2pt},
]

\node at (axis cs:0,3) [anchor=center, rotate=0] {\footnotesize{YIELD LOSS}};
\node at (axis cs:0,-3) [anchor=center, rotate=0] {\footnotesize{YIELD LOSS}};
\node at (axis cs:3,0) [anchor=center, rotate=270] {\footnotesize{ESCAPE}};
\node at (axis cs:-3,0) [anchor=center, rotate=90] {\footnotesize{ESCAPE}};
\node at (axis cs:3,3) [anchor=center, rotate=0] {\footnotesize{BAD UNIT}};
\node at (axis cs:3,-3) [anchor=center, rotate=0] {\footnotesize{BAD UNIT}};
\node at (axis cs:-3,3) [anchor=center, rotate=0] {\footnotesize{BAD UNIT}};
\node at (axis cs:-3,-3) [anchor=center, rotate=0] {\footnotesize{BAD UNIT}};

% Draw reference lines
\addplot[domain=-4:4, red, forget plot] {x};
% \addlegendentry{$y = x$}

\addplot[domain=-4:4, red, dashed, forget plot] {x + 0.4};
% \addlegendentry{$y = x + 0.5$}

\addplot[domain=-4:4, red, dashed, forget plot] {x - 0.4};
% \addlegendentry{$y = x - 0.5$}

% Positive INL points (true > 0)
\addplot[
    only marks,
    mark=*,
    mark size=1pt,
    cyan,
] table [x index=0, y index=1, col sep=space]
{Plots/StatisticalAnalysisINL/inl_statistic_pos.dat};
\addlegendentry{Positive INL}

\addplot[
    only marks,
    mark=*,
    mark size=1pt,
    purple,
] table [x index=0, y index=1, col sep=space]
{Plots/StatisticalAnalysisINL/inl_statistic_neg.dat};
\addlegendentry{Negative INL}

\end{axis}
\end{tikzpicture}
